Taking a Deeper Look at the Inverse Compositional Algorithm

In this paper, we provide a modern synthesis of the classic inverse compositional algorithm for dense image alignment. We first discuss the assumptions made by this well-established technique, and subsequently propose to relax these assumptions by incorporating data-driven priors into this model. More specifically, we unroll a robust version of the inverse compositional algorithm and replace multiple components of this algorithm using more expressive models whose parameters we train in an end-to-end fashion from data. Our experiments on several challenging 3D rigid motion estimation tasks demonstrate the advantages of combining optimization with learning-based techniques, outperforming the classic inverse compositional algorithm as well as data-driven image-to-pose regression approaches.

==> srcs/applications.tex <==
\section{Learning Robust 6D Transform}
\label{sec:learning_6d_transform}

\noindent \textbf{Direct Methods for 3D Motions} We treat the egocentric or allocentric motion estimation as a general 6D motion and apply our direct methods to solve it without specific treatments. The input is two RGB-D frames given the camera intrinsics, and no other information are available at inference time. Based on the actual application, the method will face different challenges, such as noisy depth from active sensor or stereo, significant occlusions, inconsistent texture shading and large motions. We expect the same algorithm can adapt to all various challenges driven only by the training data.

\noindent \textbf{Entangled Object Pose Estimation} \zlnote{Not finished yet. Will update on KITTI experiments.}  To estimate all rigid motions $\xi^{i} \in \se{3}, i \in \{1,2,...,N\}$ given detected $N-1$ objects and the camera itself. The correct association of every object across frames should emerge from the estimated relative motion. 

%We assume that an object can be detected through appearance by the state-of-art object detector on the reference frame, which will include both static and dynamic objects. No instance association across frames are known.



==> srcs/deep_models.tex <==
\section{Learning Direct Method}

We propose to address the drawbacks of the classical direct method by learning three light-weight modules, regarding the error modeling, inlier selection for reweighted least-square and the numerical methods to solve it.

\subsection{Overall Method}

\noindent \textbf{Inverse-compositional Least-square:} We use the classical inverse-compositional (IC) form \cite{Baker04ijcv} to model the nonlinear-least square problem. At iteration $k$, the objective is to solve an origin perturbed transform $\delta \xi \in \se{3}$, by minimizing total residual $\residual(\pixel, \delta \xi;\xi_{k-1})$ on the image space. In the following notations, we will represent it as $\residual^{k}(\delta \xi)=\residual(\pixel, \delta \xi;\xi_{k-1})$ and drop all $\pixel$for simplicity. 
\begin{align} \label{eq:IC_objective}
\argmin_{\delta \xi} &\sum_{\pixel \in \domain} \residual^{k}(\delta \xi)^{\top}  \weight^{k}(\theta_\weight) \residual^{k}(\delta \xi) \\
\residual^{k}(\delta \xi) &= \descriptor{\text{ref}}{\delta \xi;\theta_C} - \descriptor{\text{trg}}{\warp(\xi_{k-1});\theta_{C})}
\end{align} 
\noindent \textbf{Trust-region update:} An optimal solution at each iteration can be analytically calculated using the trust-region update: 
\begin{align} \label{eq:IC_update}
\xi^{\star} = -\sum_{\pixel}(\jacobian^{\top}\weight^{k}(\theta_\weight)\jacobian + \lambda(\theta_\lambda)\identity)^{-1}\jacobian^{\top}\weight^{k}(\theta_\weight)\residual^{k} 
\end{align} 

\noindent \textbf{Three networks:} we use $\descriptor{i}{\cdot;\theta_{C}}$ to represent the network that learns the feature, $w^{k}(\theta_\weight)$ for robust weighting and $\lambda(\theta_{\lambda})$ for optimal trust-region damping.

After each update, we use the inverse update on $\xi_{k-1}$ that $\xi_{k}= -\delta_\xi \composite \xi_{k-1}$ using Rodrigues' formula. The benefit of using the IC form is that we can pre-compute the origin perturbed Jacobian $\jacobian$ and reused it for each iteration \footnote{See supplmentary materials for details of Jacobians derivation}: 
\begin{align}
\jacobian &= \frac{\partial \descriptor{\text{ref}}{\pixel;\theta_{c}}}{\partial \pixel} \frac{\partial \warp(\pixel,\xi;\zero)}{\partial \xi}
\end{align}

\noindent \textbf{Overall Method:} We summarize the steps of one trust-region update in Fig.\ref{fig:trust-region-pipeline}. There are three iterations in each pyramid level and a total of four pyramids from coarse-to-fine. At training time, we only need the supervision from the optimal solutions and all the modules with learnable weights are adjusted. At inference time, the method perform the iterative estimation with fixed weights iteratively following Eq.\ref{eq;IC_update}. 

\noindent \textbf{Coarse-to-fine Trust-region Iterations} Since the origin perturbed linearization of Eq.\ref{eq:IC_objective} hold on its local manifold, computing the iteration coarse-to-fine on the pyramids reduces the necessary number of iterations to reach global optimum in theory. In this work, we use a fixed setting of four pyramids scales. And optimazation on each scale use the initialized value from the last iteration.

\subsection{Learning Error Modeling} 
\label{sec:feature_net}

The feature moduel $\descriptor{\text{ref}}{\cdot;\theta_{C}}$ concatenate the reference frame with the target frame RGB-D (inverse depth) as input, and output a pyramid (of four) features across four-scales as output. At each pyramid, the network use a three dilated convolutional layers with dilation [1,2,4] \zlnote{Need a table to summary all the network parameters} and shrink the pyramid to half by spatial average pooling. We keep the output feature map channel dimension constant at one by channel-wise sum the corresponding features. Different from the other methods that learn a multi-dimensional feature space for residual estimation \cite{Wang18cvpr}, our proposed method has two novel properties:

\noindent \textbf{Efficient compound residuals} We output a one-channel feature image from different sources (RGB-D) which can be applied to a single residual function and weighting function. Since the channel dimension is only 1, it also makes the training and inference fast.\ag{sure, but don't you loose accuracy?}

\noindent \textbf{Informative gradients for image Jacobian} In the traditional Direct Method, the Jacobian is only calculated on the reference image, which is not able to adapt to various motion types. To enable the network learn more informative image gradient for different challenges, we propose to concatenate the reference image with the target image. We find it significantly help the network to learn a geodesic measure when the warped target image has large displacement to the reference image. \zlnote{Mayne needs an example image to show the effects of large motions?}

\subsection{Convolutional M-estimator}
\label{sec:CM-est}

We propose the \emph{convolutional M-estimator (CM-est)} which estimates the weighted residual with a learned weighting function from data, as shown in the Fig. \ref{fig:deep_m-estimator}. Inspired by the traditional M-estimator discussed in Sec.\ref{sec:reweighted_least_square}, we take the residual as input, together with relevant feature information as context. 

The deep M-estimator is composed of three layers dilated conv-net and followed by a sigmoid layer which normalizes the weighted function to the range of $[0,1]$. This module works as the attention \cite{Vaswani17nips} of an optimizer, which weights the data driven by the ground truth optimal solutions. 
 
Different from \cite{Ranftl18eccv} which only needs a one-shot weight prediction from a set of sparse points, our residuals need to be frequently evaluated spatially on each pixel. To reduce the number of residual evaluation, which can be quite heavy in our residual volumes, we propose to only calculate $\weight_{k}$ once based on the input residual $\residual_{k-1}$. 

\subsection{Learning the Trust Region}
\label{sec:DTM}

\zlnote{Currently we have several forms of the trust-region methods and which way is in favor will depend on the experiments these days. Will converge on this section very soon. And this section has some legacy content to be updated.}

\noindent \textbf{Residual Volumes from Damping Proposals:} Inspired by the success of Cost-volume \cite{Dosovitskiy15iccv,Sun18cvpr} and Plane-sweeping stereo \cite{Flynn16cvpr}, we propose to approximate the trust-region update in Sec.\ref{sec:trust_region_method} by sampling several proposals first according to Eq.\ref{eq:reweighted_LS_manifold} and concatenate the spatial residuals of each sampled update into one residual volume $\residual_{i}(\delta \xi_{i}), i\in\{1,2,...M\}$. This residual volume indicates the attention for the fastest convergence route to minimum residuals. Instead of randomly sampling the proposals of $\lambda$, we first calculate the largest eigen-value $\lambda_{max}$ of the approximate Hessian $\jacobian^{\top}\jacobian$, and then sample 25 proposals of the damping $\lambda$ in log scale between $[\lambda_{max}/1e4, \lambda_{max}\cdot1e2]$. According to this sampling distribution, the Hessian is regularized to be well-conditioned \ag{say why} and the diagonal damping is approximately uniform distributed \ag{within what?}. With a well conditioned Hessian, we can also analytically derive its gradient of its inverse function. Note each Hessian only has a dimension of $6\times6$, which can be much more efficiently computed on CPU threads than on the GPU kernels.

\noindent \textbf{Damping Prediction:} From the weighted residual volume, we use a global average pooling layer to compress it into a residual vector. We uses two strategies in estimating damping. The first approach uses a \emph{Soft Argmin} operation \cite{Kendall17iccv} to estimates the optimal damping from the weighted samples, which is parameter-free. The second approach regress the damping from the residual factor using two layers of fully connected (\emph{FC}) layers. Both methods can lead to reasonable damping with good generalization. We will show a comparison of both in Sec.\ref{sec:experiments}. \ag{too imprecise. make it formal}

%\begin{figure}[t!]
%	\centering 
%	\includegraphics[width=\linewidth]{deep_trust_region_method} 
%	\caption{One step update of Deep Trust-Region Method. Given the reference frame feature $\feature_0$, depth $\depth_0$ and the residual in both $\residual^{\feature}, \residual^{\depth}$, we can pre-compute the weights $\weight$ (for residual) and the Jacobians $\jacobian$. At each iteration, we sample the damping proposals $\lambda_i$ and calculates the residuals with the proposed updates. Finally the damping prediction layer will calculate the optimal damping $\lambda^{\star}$ from which we calculate the optimal solution in that step.}
%	\label{fig:trust-region-pipeline}
%\end{figure}

\input{srcs/training}

%\section{Deep Robust Object Scene Flow}
%
%We focus on the scene flow problem observed from a moving camera and multiple moving objects can appear. The input is two RGB-D frames given the camera intrinsics, and no other information are available. We assume that an object can be detected through appearance by the state-of-art object detector on the reference frame, which will include both static and dynamic objects. No instance association across frames are known. Our goal is to estimate all rigid motions $\xi^{i} \in \se{3}, i \in \{1,2,...,N\}$ given detected $N-1$ objects and the camera itself. The correct association of every object across frames should emerge from the estimated scene flow.
%
%\noindent \textbf{Train} We supervise the training of the object scene flow network with ground truth two-view transform. At training time, we randomly sample at object with its bounding box as ROI. In reference frame, all residuals outside of the ROI are markable as zero.  %\cite{Li18eccv}


==> srcs/formula_backup.tex <==
Since the seminal paper of Lucas and Kanade \cite{Lucas1981IJCAI} from 1981, dense image alignment has become a ubiquitous tool in computer vision with many applications including tracking \cite{tbd}, pose estimation \cite{tbd}, image registration \cite{tbd} and dense SLAM \cite{tbd}.
The basic idea behind the original Lucas-Kande algorithm is 
to minimize the photometric error between a template $\bT\in\nR^{W\times H}$ and an image $\bI\in\nR^{W\times H}$ by warping the template towards the template:
%
\begin{equation}
\min_{\bxi} \sum_{\bx\in\Omega}{\Vert \bI(\cW(\bx;\bxi)) - \bT\Vert}_2^2
\label{eq:lk_objective}
\end{equation}
%
Minimizing \eqref{eq:lk_objective} is a non-linear optimization task as the image $\bI$ depends non-linearly on the pixel locations $\bxi$.
Thus, the Lucas-Kanade algorithm iteratively solves for parameter increments $\Delta \bxi$.
%
\begin{equation}
\min_{\bxi} \sum_{\bx\in\Omega}{\Vert \bI(\cW(\bx;\bxi+\Delta\bxi)) - \bT\Vert}_2^2
%\min_{\Delta\bxi} {\Vert \bI(\bxi+\Delta\bxi) - \bT\Vert}_2^2
\label{eq:lk_iterative}
\end{equation}
%
updating $\bxi \gets \bxi + \Delta \bxi$ at every iteration, linearizing \figref{eq:lk_iterative} using first-order Taylor expansion
%
\begin{equation}
\min_{\Delta\bxi} \sum_{\bx\in\Omega}{\Bigg\Vert\bI(\cW(\bx;\bxi)) + \frac{\partial \bI(\cW(\bx;\bxi))}{\partial \bxi} \Delta\bxi - \bT\Bigg\Vert}_2^2
\label{eq:lk_linearized}
\end{equation}
%
where the steepest descent image $\partial \bI(\bxi)/\partial \bxi$ is the composition of image gradients and the warp Jacobian.


















\section{Introduction}

Since the seminal paper of Lucas and Kanade \cite{Lucas1981IJCAI} from 1981, dense image alignment has become a ubiquitous tool in computer vision with many applications including tracking \cite{tbd}, pose estimation \cite{tbd}, image registration \cite{tbd} and dense SLAM \cite{tbd}.
The basic idea behind the original Lucas-Kande algorithm is 
to minimize the photometric error (residual) between a template $\bT\in\nR^{W\times H}$ and an image $\bI\in\nR^{W\times H}$ by warping the image towards the template:
%
\begin{equation}
%\min_{\bxi} {\Vert \bI(\bxi) - \bT\Vert}_2^2
\min_{\bxi} {\Vert \br(\bxi)\Vert}_2^2 \quad \text{with} \quad \br(\bxi) = \bI(\bxi) - \bT
\label{eq:lk_objective}
\end{equation}
%
Minimizing \eqref{eq:lk_objective} is a non-linear optimization task as the image $\bI$ depends non-linearly on the pixel locations $\bxi$.
Thus, the Lucas-Kanade algorithm iteratively solves for parameter increments $\Delta \bxi$.
%
\begin{equation}
%\min_{\Delta\bxi} {\Vert \bI(\bxi+\Delta\bxi) - \bT\Vert}_2^2
\min_{\Delta\bxi} {\Vert \br(\bxi+\Delta\bxi)\Vert}_2^2
\label{eq:lk_iterative}
\end{equation}
%
updating $\bxi \gets \bxi + \Delta \bxi$ at every iteration, linearizing \figref{eq:lk_iterative} using first-order Taylor expansion
%
\begin{equation}
%\min_{\Delta\bxi} {\Bigg\Vert\bI(\bxi) + \frac{\partial \bI(\bxi)}{\partial \bxi} \Delta\bxi - \bT\Bigg\Vert}_2^2
\min_{\Delta\bxi} {\Bigg\Vert\br(\bxi) + \frac{\partial \bI(\bxi)}{\partial \bxi} \Delta\bxi\Bigg\Vert}_2^2
\label{eq:lk_linearized}
\end{equation}
%
where the steepest descent image $\partial \bI(\bxi)/\partial \bxi$ is the composition of image gradients and the warp Jacobian. In this \textit{forward compositional} formulation, the steepest descent image needs to be recomputed at every iteration as it depends on $\bxi$. In contrast, the \textit{inverse compositional} algorithm \cite{Baker2001CVPR,Baker2002} reformulates \eqref{eq:lk_objective} by warping the template instead of the image:
%
\begin{equation}
%\min_{\bxi} {\Vert \bI(\bxi) - \bT\Vert}_2^2
\min_{\bxi} {\Vert \br(\bxi)\Vert}_2^2 \quad \text{with} \quad \br(\bxi) = \bI - \bT(\bxi)
\label{eq:ic_objective}
\end{equation}
%
This leads to an interative update
%
\begin{equation}
%\min_{\Delta\bxi} {\Bigg\Vert\bI(\bxi) + \frac{\partial \bI(\bxi)}{\partial \bxi} \Delta\bxi - \bT\Bigg\Vert}_2^2
\min_{\Delta\bxi} {\Bigg\Vert\br(\bxi) + \frac{\partial \bT(\bxi)}{\partial \bxi} \Delta\bxi\Bigg\Vert}_2^2
\label{eq:ic_linearized}
\end{equation}
%
in which 

%The most time-consuming step of this \textit{forward compositional} algorithm is the computation of the steepest descent  which needs to be re-evaluated at every iteration as it depends on $\bxi$.

%, can be pre-computed.


%is minimized with respect to the parameters of the warping function using non-linear optimization.
%Algorithms for dense image alignment can be categorized as either \textit{additive} or \textit{compositional}, and as either \textit{forwards} or \textit{inverse} \cite{Baker2001CVPR,Baker2002}.
%The inverse compositional algorithm is appealing as the most time-consuming step, the computation of the Hessian, can be pre-computed.


%There are two major formulations 
%Thereby, the warping function is parameterized b
%There exist two major paradigms for image alignment
%\cite{Baker2001CVPR,Baker2002}

% applications

% later mention generalization to 3D, instances, etc.

==> srcs/overall_method_fig.tex <==
\begin{figure*}
	\centering 
	\subfloat[][The iterative coarse-to-fine linearized update for direct method ]{\includegraphics[width=0.9\textwidth]{overviews/overall_flowchart} \label{fig:overall_method}} \\
	\subfloat[][The inverse compositional update in one trust region iteration]{\includegraphics[width=0.9\textwidth]{overviews/ic_update}\label{fig:ic_update}}
\caption{The overall flow-chart of our algorithm }
\end{figure*}

==> srcs/preliminaries.tex <==
\section{Preliminaries}

Solving for the rigid transform $T(\xi) \in \M{4\times4}, \xi \in \se{3}$ given two frames can be formulated as a nonlinear optimization problem. We will describe the general approach first. Then we will see the limitations in traditional approaches and how we propose to solve it.

\subsection{Error Modelling}
\label{sec:error_modeling}

In general, the classical direct method models the residuals of two images regarding the relative transform. For all pixels $\pixel \in \Omega$, given an estimated warping $\warp(\pixel;\xi)$ regarding an unknown transform $\xi \in \se{3}$, the residuals $\residual(\pixel) \in$ on reference image to the wapred target image is:
\begin{align}\label{eq:residual_model}
\residual(\pixel;\xi) = \descriptor{\text{ref}}{\pixel} - \descriptor{\text{trg}}{\warp(\pixel;\xi)} 
\end{align}
\noindent \textbf{Differentiable Image Descriptors:} $\descriptor{i}{\pixel}$ is the descriptor on the $i$th image.
The classical direct method parameterize $\descriptor{i}{\pixel}$ using intensity image \emph{brightness-consistency} assumption, or using depth to check the reprojection error. To better model the invariance in the image space, recently work measure the residual distance on more abstract descriptor space, e.g. SSIM \cite{Wang04tip} or differentiable Census \cite{Lv16eccv}. Here we use $\residual(\pixel)$ to represent the residuals assembled from different sources $\residual_{i}(\pixel)$.

Estimating the optimal $\xi$ can be solved as maximum a posteriori (MAP) problem. ML estimation is naturally robust in itself if the we can model the residuals correctly \cite{Triggs99iwva} for the pixel-wise information, which however is a nontrivial problem in itself. \zlnote{Have not talked about the problem of the loss yet. Aperture, photometric inconsistence, etc. }

\subsection{Iterative Re-weighted Least-square (IRLS)}
\label{sec:reweighted_least_square}

A general framework to solve the MAP problem is via re0weighted least-square estimation, which iteratively solve the following objective with a symmetric positive-definite weight matrix $\weight(\pixel)$ at each $\pixel$:
\begin{align}
\label{eq:reweighted_least_square}
\energy(\xi) = \frac{1}{2} \sum_{\pixel \in \Omega}\residual(\pixel;\xi)^{\top}\weight(\pixel)\residual(\pixel;\xi)
\end{align}
\noindent \textbf{M-estimators:} $\weight(\pixel)$ is a block-diagnol matrix for the compound residuals as $\weight(\pixel)=\text{Diag}(\weight_1(\pixel),...,\weight_k(\pixel))$. A popular family of modeling $\weight_{i}(\pixel)$ is called M-Estimators \cite{Black96cviu}, which models the statistical distributions of residuals with a \emph{predefined} statistical model and weight the residual $\residual_{i}(u)$ in each iterative update.

Although the favorate chosen M-estimators are statistically driven, they can ensure the optimality of inlier selection only if the correct inlier distribution can be pre-defined. However, when the initial estimation is not close to its optimal solution or there are significant outliers that cause the ambiguity, its inappropriate weighting will lead to sub-optimal solutions.

\subsection{Numerical Method}
\label{sec:trust_region_method}

\zlnote{The following residual annotation is not consistent with the above. We will use a whitened residual here. Will fix...}
One classical approach to estimate the optimum $\xi^{\star}$ is to linearize Eq. \ref{eq:reweighted_least_square} and iteratively minimize the quadratic model, with an initial value of $\xi_{k}$ at the $k$th iteration:
\begin{align}
\label{eq:trust_region_method}
\xi^{\star} = \argmin_{\xi} \norm{\residual^{w}_{k}}_2 &+ \xi^{\top}\jacobian^{\top}\residual^{w}_{k} + \frac{1}{2} \xi^{\top} (\jacobian^{\top} \jacobian + \lambda \eye) \xi \\
s.t. ||\xi|| &\leqq \Delta_{k}
\end{align}

where $\residual^{w}_{k}=\weight \Hadamardproduct \residual(\xi_{k}) \in \M{N\times1}$ for simplicity. $\jacobian$ is the Jacobian matrix that $\jacobian=\partial(\weight \Hadamardproduct \residual(\xi))/\partial \xi \in \M{N\times6}$. $\lambda \eye$ is the damping function which regularize the approximate weighted Hessian $\jacobian^{\top}\jacobian$ and $\Delta_{k}$ is the trust-region. The solution of this constrained problem is the solution of: 
\begin{align}
\label{eq:trust_region_update}
(\jacobian^{\top}\jacobian + \lambda \eye) \xi^{\star} = -\jacobian^{\top} \residual^{w}_{k}
\end{align}

\noindent \textbf{Trust-region Method:} When $\lambda$ varies, the optimal solution $\xi^{\star}$ varies between the direction along the Newton direction $-(\jacobian^{\top}\jacobian)^{-1}\jacobian^{\top}$ (when $\lambda=0$) and negative gradient search $-1/\lambda \cdot \jacobian^{\top}$ (when $\lambda \rightarrow \infty$). In general, the family of trust-region methods converge by iteratively evaluating residuals and changing its damping on-the-fly, with different heuristic rules. An example of the most well-known of them $\lambda$-parameterized Levenberg-Marquardt use the following heuristic :

% write a more rigorous classical Levenberg Marquart algorithm
\begin{description}[noitemsep,nolistsep,leftmargin=*]
	\item[Update and evaluate:] $e=\energy(\xi)$ in Eq. \ref{eq:reweighted_least_square}. 
	\item[If $e$ increases, increase $\lambda$:] reset the steps, and increase $\lambda$ \eg by a factor of 10. Try update and evaluate again.
	\item[If $e$ decreases, accept:] move to the next iteration and decrease $\lambda$ \eg by a factor of 10. 
\end{description}

The damping $\lambda$ found through the above update rule is heuristic and not optimal for any well defined criterion. It is widely accepted because it empirically works well, compared to other classical technics. In a cluttered environment with inputs using natural images or noisy depth, the solution of the trust-region methods with minimum residuals may not match the ideal optimum at all, under heavy occlusion, inconsistent shading, sensor noise, and bad initial guess. Traditionally, people treat the optimization as an independent process and try to pre-process the inputs and outliers carefully by incorporating hand-crafted assumptions or object-based priors. Unfortunately, none of these efforts can generalize the motions in the wild.

%\noindent \textbf{Integrate Priors into Trust-region Methods} From Eq. \ref{eq:trust_region_update}, the optimal update can be influenced by the damping $\lambda$ and the weight function $\weight$. $\weight$ can indirectly affect $\residual^{w}_{k}$ and $\jacobian$. Choosing either $\lambda$ or $\weight$ smartly requires prior knowledge, which can be learned through data. Potentially, the resistance to occlusion, noise, shading and motion ambiguity can be represented in $\weight$ as a confidence per datum. Suppose the learned prior can help the optimizer find a better update direction, which can converge within minimum steps even for very large motions. An intuition of it is shown in Fig.\ref{fig:trust-region-intuition}. We can even accelerate the convergence speed with traditional pyramid updates, shown in Fig.\ref{fig:coarse-to-fine-trust-region-search}. 

%\begin{figure*}[h!]
%	\centering
%	\subfloat[Trust-region Intuition.]{
%		\includegraphics[width=0.25\textwidth]{trust-region-intuition} 
%		\label{fig:trust-region-intuition} 
%	} 
%	\subfloat[Coarse-to-fine Trust Region Search Intuition. ]{
%		\includegraphics[width=0.4\textwidth]{coarse-to-fine} 
%		\label{fig:coarse-to-fine-trust-region-search} 
%	} 
%%	\subfloat[Coarse-to-fine Trust Region Update]{
%%		\includegraphics[width=0.3\textwidth]{coarse-to-fine-trust-region} 
%%		\label{fig:coarse-to-fine-trust-region-diagram} }
%	\\
%	\caption{(a) The trust-region method solves the motion in its parameter space. Suppose there is an optimal update $\xi^{\star}$ between the negative gradient direction $-1/\lambda \cdot \jacobian^{\top}$ and Newton's direction $-(\jacobian^{\top}\jacobian)^{-1}\jacobian^{\top}$. Instead of searching for the optimal direction with heuristics, we can learn the searching from data. (b) Adapting the trust-region with the coarse-to-fine concept can ideally deal with large motions in finite iterations. (c) To model the coarse-to-fine trust-region, we usually perform multiple trust-region steps on the image(or feature $\feature$) pyramids. We initialize each step with the last solution.}
%\end{figure*}


==> srcs/quantitative_KITTI.tex <==
\begin{table}[]
\centering
\tiny
\begin{tabular}{@{}llllll@{}}
\toprule
                                                                                  &       &                             & 3D EPE & 2D EPE & 3D Pose \\ \midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Conv-Net \\ Single-shot\end{tabular}}  & (c-1) & RGBD                        &        &        &         \\
                                                                                  & (c-2) & RGBD (Compact)              &        &        &         \\ \midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Learn \\ Direct\\ Method\end{tabular}} & (I-1) & No learning                 &        &        &         \\
                                                                                  & (l-2) & Two-view FN                 &        &        &         \\
                                                                                  & (l-3) & Two-view FN + FCM-Est       &        &        &         \\
                                                                                  & (I-4) & Two-view FN + FCM-Est + DTM &        &        &         \\ \bottomrule
\end{tabular}
\caption{\textbf{Quantitative evaluations on KITTI 6D} }
\label{tab:kitti_quantitatve}
\end{table}

==> srcs/quantitative_refresh.tex <==
\begin{table*}[]
	\centering
	\tiny
\begin{tabular}{@{}lllcccccccccc@{}}
	\toprule
	& \multirow{2}{*}{ID} & \multicolumn{1}{c}{\multirow{2}{*}{Model Descriptions}} & \multicolumn{4}{c}{3D EPE (m) Validataion/Test}                                           & \multicolumn{4}{c}{Test  t \textless 5 cm \& R \textless 15 deg}                          & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Model \\ Parameters\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Inference \\ Time\end{tabular}} \\ \cmidrule(lr){4-11}
	&                     & \multicolumn{1}{c}{}                                    & KF 1                 & KF 4                 & KF 8                 & KF 16                & KF 1                 & KF 4                 & KF 8                 & KF 16                &                                                                              &                                                                            \\ \midrule
	\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Traditional \\ Direct \\ Method\end{tabular}} & (t-1)               & Two-view Intensity (ours no learnable parameter)        & -/0.102              & -/0.307              & - /0.443             & -/0.61               &                      &                      &                      &                      &                                                                              &                                                                            \\
	& (t-2)               & RGBD VO \cite{Steinbrucker11iccvw} (Open3D\cite{Zhou18arXiv} Implementation)                                        &                      &                      &                      &                      &                      &                      &                      &                      &                                                                              &                                                                            \\
	& (t-3)               & Point-Plane ICP \cite{Chen92ivc} (Open3D\cite{Zhou18arXiv} Implementation)                               &                      &                      &                      &                      &                      &                      &                      &                      &                                                                              &                                                                            \\ \midrule
	\multirow{2}{*}{Conv-Net}                                                                & (c-1)               & RGBD +1 Iteration                                       &                      &                      &                      &                      &                      &                      &                      &                      & 7154                                                                         &                                                                            \\
	& (c-4)               & Compact Net: RGBD + 1 Iteration                         &                      &                      &                      &                      &                      &                      &                      &                      &                                                                              &                                                                            \\ \midrule
	\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Learn \\ Direct\\ Method\end{tabular}}                                                     & (l-1)               & Two-view FN                                             &                      &                      &                      &                      &                      &                      &                      &                      &                                                                              &                                                                            \\
	& (l-2)               & Two-view FN + FCM-Est                                   & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}                                                         & \multicolumn{1}{l}{}                                                       \\
	& (I-4)               & Two-view FN + FCM-Est + DTM                             & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}                                                         & \multicolumn{1}{l}{}                                                       \\ \bottomrule
\end{tabular}
\caption{\textbf{Quantitative evaluations on ego-centric estimation using BundleFusion \cite{Dai17tog} with dynamic humans rendered in RefRESH\cite{Lv18eccv}. }}
\label{tab:refresh_quantitative}
\end{table*}

==> srcs/teaser_image.tex <==
\begin{figure}
	\centering 
	\includegraphics[width=\linewidth]{mask_rcnn_example_000199_10} 
	\caption{Multiple instance 3D motion estimation using our proposed learned Direct Method \zlnote{Currently only results from mask-rcnn.  We will add a 3D visualization of their estimation motions here. Weclome to give suggestions about visualization.}}
	\label{fig:teaser}
\end{figure}

==> srcs/training.tex <==
\subsection{Train the Deep Direct Method}

\noindent \textbf{Training Loss} We use the Point Matching Loss as \cite{Li18eccv} to balance the translation and rotation. We convert the reference image depth $\depth(\pixel)$ into a point cloud $\point(\pixel)$ with the camera intrinsics. Given the ground truth transform $[\rotation_{\text{gt}}, \translation_{\text{gt}}]$ and the estimated $[\rotation_{\text{est}}, \translation_{\text{est}}]$, we calculate the matching error at each pyramid:

\begin{equation}
\loss = \sum_{\pixel \in \Omega} \norm{(\rotation_{\text{est}} \point(\pixel) + \translation_{\text{est}}) -  (\rotation_{\text{gt}} \point(\pixel) + \translation_{\text{gt}})}
\end{equation}

We apply the loss function with equal weights to the intermediate solutions from each coarse-to-fine pyramid.

\noindent \textbf{On the numerics of inverse Hessian} Although the matrix inverse operation is differentiable, we find this process can cause several numerical problems as floating point operation which need to be carefully addressed. Depending on the image size, we may count millions of accumulated residuals which make the scale of the Hessian $\hessian$ very large, leading to inaccurate inverse operation and gradients. To address this, we normalize $\hessian'=\hessian/M$ and accumulated residual $\residual'=\residual/M$ which $M$ is the mean of $\residual$. We use the pseudo-inverse of the Hessian in the training.


